Applied Similarity Problems Using Frechet Distance

In the first part of this thesis, we consider an instance of Frechet distance problem in which the speed of traversal along each segment of the curves is restricted to be within a specfied range. This setting is more realistic than the classical Frechet distance setting, specially in GIS applications. We also study this problem in the setting where the polygonal curves are inside a simple polygon. In the second part of this thesis, we present a data structure, called the free-space map, that enables us to solve several variants of the Frechet distance problem efficiently. Our data structure encapsulates all the information available in the free-space diagram, yet it is capable of answering more general type of queries efficiently. Given that the free-space map has the same size and construction time as the standard free-space diagram, it can be viewed as a powerful alternative to it. As part of the results in Part II of the thesis, we exploit the free-space map to improve the long-standing bound for computing the partial Frechet distance and obtain improved algorithms for computing the Frechet distance between two closed curves, and the so-called minimum/maximum walk problem. We also improve the map matching algorithm for the case when the map is a directed acyclic graph. As the last part of this thesis, given a point set S and a polygonal curve P in R^d, we study the problem of finding a polygonal curve Q through S, which has a minimum Frechet distance to P. Furthermore, if the problem requires that curve Q visits every point in S, we show it is NP-complete.

==> Conclusion/Conclusion-Open_New.tex <==


\chapter{Conclusions and Open Problems}
\label{ch:OpenProblems}

As the first part of 
this thesis, we introduced 
a new generalization of the well-known \Frechet distance between two polygonal
curves, and provided an efficient algorithm for computing it. In our  variant of the \Frechet problem, the speed of 
traversal along each segment of the curves is restricted to be within a specified range. This setting is more realistic than the classical \Frechet distance setting, specially in GIS applications.
We presented an efficient algorithm to solve the decision problem
in $O(n^2 \log n)$ time, which together with a  parametric search,
led to an $O(n^2 \log^2 n)$ time algorithm for finding 
the exact value of the \Frechet distance with speed limits.
We also studied speed-constrained \Frechet distance in the case where the curves
are located inside a simple polygon.
Several open problems arise from our 
work.
It is interesting to consider speed limits in other variants of the \Frechet distance studied in the literature,
such as the \Frechet distance between two curves lying 
on a convex polyhedron~\cite{AnilFrechet}, or on a polyhedral surface~\cite{WenkC08a}. 

Another open problem in the context of 
part I of the thesis is whether 
our results can be applied in matching planar maps, where the objective is 
to find a path in a given road network that is as close as possible to a vehicle trajectory. 
In~\cite{AltERW03a}, the traditional \Frechet metric is used to match 
a trajectory to a road network. 
If the road network is very congested,  
the \Frechet distance with speed limits introduced in this thesis seems to find a more realistic path in the road network, 
close to the trajectory of the vehicle.
It is also interesting to extend our variant of the \Frechet distance 
to the setting where the speed limits on the segments of the curves change as functions over time.


In the second part of this thesis, 
we introduced a data structure, 
called free space map, which can be used 
as an alternative to the free-space diagram 
in applications related to 
\Frechet distance. 
Our has the same size and construction time as the standard
free-space diagram, and 
encapsulates all the information available in that diagram, 
yet it is capable of answering a more general type of queries efficiently. 
One major open problem in the 
context of Part II of the thesis
is whether one could construct 
a balanced binary search 
tree on top of free-space map, 
to quickly answer dynamic queries such as:
removing some vertices from the input curves 
or adding some new 
vertices to the curves, how fast 
we could solve decision problems or
recompute \Frechet distance.
\REM{
In the following, we explain the difficulty of constructing such data structure: 



There are several interesting dynamic problems related to \Frechet metric
that to our knowledge, have not yet been addressed  in the literature:


Let  $P$ and $Q$ be 
two polygonal curves of length $n$ and $m$, respectively.
By spending $O(nm \log nm)$  , one can compute the \Frechet distance between   $P$ and $Q$ (i.e. $\distF(P,Q)$). 
Now, we want to know how fast we can recompute $\distF(P,Q)$, after:
  splitting some edges of $P$ (resp., $Q$),
  or deleting some vertices  of polyline $P$ (resp., $Q$),
  or merging some consecutive vertices of $P$ (resp., $Q$) into one vertex. 


%A curve $P$ and and a segment $S$ are given.
%Let $Q$ be the curve achieved by  
%putting a point $p$ on the perpendicular bisector of $S$ and connecting two end-points of $S$ to $p$. The point $p$ should be chosen  in a way that optimizes the \Frechet distance between $P$ and $Q$. 
%
%Curve Refinement (Version 1.) Given curve $P$ and $Q$.
%Delete one node ( or some nodes ) from $Q$ to achieve a new curve $Q'$ 
%s.t. $\delta(P,Q')$ is minimized.
%(Version 2.) Curve $P$ and $Q$ are given. We would like to delete some nodes from $Q$ s.t. the deletion has the least  impact on the \Frechet distance between $P$ and $Q$.


%The free space diagram $\BNM$ (See Figure~\ref{fig:diagram}) is  a data structure 
%proposed by Alt \etal ~\cite{AltG95}  to solve the decision problem of \Frechet metric.
%We want to design another data structure on top of the free space diagram with which 
%answering the decision problem of \Frechet metric takes less than $O(mn)$ time.
%(after constructing that data structure). 

Consider the free-space diagram $\BNM$ corresponding to curves $P$ and $Q$, and input parameter $\epsilon \ge 0$.
Let $\row{i} = \Feps \cap y = i, i \in \{1,\dots,m+1\}$. 
%Also, let a {\em feasible} interval $I$ be a maximal connected set of white points on the bottom side of a cell.
Notice that given an arbitrary point $p \in \row{i}$, the number of intervals in $\row{j}$, $j > i$, which are monotonically reachable from $p$, 
is linear in the number of cells in one row. 
Let $\RSet{i}{j}$ denote the set of intervals in $\row{j}$ which are reachable from 
every point $p \in \row{i}$. We observed that for any $i$ and $j$, $j>i$, 
$\RSet{i}{j}$ has linear complexity (proportional to the number of cells in a row of $\BNM$). 
We store the reachability information in $\BNM$ in a data structure 
called {\em free space tree} in order to quickly update that information 
after performing the above operations. 

%We say a point $q \in \row{j}$ is monotonically reachable from a feasible interval $I \in \row{i}$, $i<j$, if it's reachable from some points in $I$. 
%Let $\BR_{ij}(I)$ be the maximal set of points in $\BF_{ij}$ reachable from an interval $I \in \row{k}$, $k<j$.

%A set $\RSet{i}{j} = \bigcup_{r=1}^{n}{\BR_{rj}(I)}, j>i,$ where $I$ can be any feasible interval in  $\row{j}$, is called the {\em reachability set} of $i^{th}$ row on the $j^{th}$ row. 

%Assume that we split $\BNM$ in half to two diagrams $D_1$ and $D_2$






The free space tree is a balanced binary search tree, denoted by $T_{\epsilon}$, 
which we construct on the top 
of the free-space diagram (See Figure \ref{fig:freeSpaceTree}.a). 
Each leaf $v_i$ in the tree corresponds to $\row{i}$ and
stores  reachability set $\RSet{i}{i+1}$.
%Two leaves $v_i$ and $v_{i+1}$, $i \in \{ 1,3,5 \dots m-1\}$ are connected to an internal node in the tree and this process is continued until the root of the tree is constructed.
%A {\em merge operation}  is the process of computing the information
%which is stored at an internal node in $T_{\epsilon}$. 
The tree is built bottom-up from the leaves to the root:
at an internal node $w$, with leaf $v_i$ as the left child
and leaf $v_j$ as the right child, the reachability information $\RSet{i}{i+1}$
is {\em merged} with $\RSet{j}{j+1}$ and consequently, set $\RSet{i}{j+1}$
is stored at node $w$.
The merge process is recursively continued at each internal node of the tree
by merging the reachability information stored at the left and right child of 
that node, until the root of the tree is reached.
Likewise, at the root of the tree, 
$\RSet{1}{\floor{\frac{m}{2}}}$ (stored at the left child of the root) 
is  merged with $\RSet{\floor{\frac{m}{2}}}{m+1}$ (stored at the right child of it),
and the reachability set $\RSet{1}{m+1}$ is stored  at the root. 
Having built the tree, one can report all reachable intervals in $\row{i+1}$ from a point $p \in \row{1}$ spending $O(1) + O(k)$ time ($k$ is the number of those reachable intervals).
In fact, finding the leftmost and the rightmost point in $\row{m+1}$ reachable from $p \in \row{1}$ can be done in constant time.  



%A data structure with which we can answer the above queries in less than the
%time to recompute the \Frechet distance.
%We state 

In the following, we describe the difficulty of constructing $T_{\epsilon}$ by showing the merge at 
the root of the tree as an example of the challenge in merge operation at internal nodes 
(see Figure \ref{fig:freeSpaceTree}.b for the illustration).
Let  a {\em feasible }interval be the maximal set of white points on the bottom side of a cell. 
Assume the free-space diagram is split in half 
at $\row{\floor{\frac{m}{2}}}$. Consider a feasible interval $I_1 \in \row{\floor{\frac{m}{2}}}$ and 
two pointers $\ell_{m+1}(I_1)$ and $r_{m+1}(I_1)$, where the pointers store the leftmost and 
the rightmost point in $\row{m+1}$, reachable from some points in $I_1$, respectively. 
Imagine another feasible interval $I_2 \in \row{1}$
where  $p = \ell_{m+1}(I_2)$ and $p \in I_1$.
Now, if we could determine the leftmost point in $\row{m+1}$ reachable from $p$, then 
we would be able to determine $\ell_{m+1}(I_2)$ in constant time
and consequently, perform the merge at the root of the tree in linear time. 

Our target is to obtain a linear running time
(or near linear) for the merge operation at internal nodes. 
If we could achieve a linear merge, then we can exploit the tree for computing 
the \Frechet distance after different dynamic operations on curves. 
As an example, suppose that we delete a vertex 
from curve $Q$. This means that two rows are deleted from the free-space diagram. 
Using the free space tree, we update the reachability information 
in $O(n \log n )$ time rather than $O(n^2)$ time. Therefore, 
we could decide whether the target point in $\BNM$ is monotonically reachable or not. 
}
%This is faster than running the popular \Frechet decision algorithm which has $O(n^2)$ runtime. 

%Then, we could perform split, delete, merge or other dynamic operations 
%and then efficiently update the reachability information in the tree.
%That's what we haven't achieved yet. Figure \ref{} depicts the difficulty in merge operation. 

%
%For instance, if $\distF(P,Q)$ is known, how fast one can compute $\distF(P,Q)$
%after splitting some edges of $P$ or $Q$. More ever, 
%how fast one can compute $\distF(P,Q)$
%after splitting some edges of $P$ or $Q$.
 
\REM{
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\columnwidth]{Pics/Freespacetree2}
	\caption{ The free space tree is built on the top of the free-space diagram}
	\label{fig:freeSpaceTree}
\end{figure}
}


\REM{
We would also want to investigate about 
computing \Frechet distance in the following setting.
%\section{Weighted \Frechet Distance}
%Another interesting problem that we would like to investigate 
%is as follows. 
Consider a polygonal curve $P$ corresponding to the trajectory 
of a moving vehicle. Assume that to each edge of $P$, a parameter {\em weight}
is associated, which shows the accuracy of the sampling around that edge.
Our goal is to compute the \Frechet distance between two curves 
taking into consideration the weights on the edges. 
%This setting might find many practical applications in GIS.
In this setting, the free space inside each cell in the free-space diagram 
corresponding to the curves, shrinks. To solve the decision problem, 
one needs to first discover the properties of the free space inside each cell, 
whether it is convex or $xy$-monotone or if it is connected or not. 
Next, the boundary of the free space inside the cells must be computed.
Finally, the free-space diagram is searched to find a monotone path from the bottom-left corner to the top-right corner. 
}

%In this setting, the distance measure between two points $a \in P$ and $b \in Q$ 
%is multiplied by the weight of the edge which point $a$ belongs to.



%
%Vehicle tracking data is an essential “raw” material
%for a broad range of applications such
%as traffic management and control, routing,
%and navigation. An important issue with this
%data is its accuracy.


%\newpage
In the third part of this thesis, 
we introduced a new variant of
\Frechet distance problem, 
called Curve-Pointset (CPM) Problem, and showed that
given a polygonal curve $P$ of $n$ segments and a set $S$ of $k$ points in $\IR^d$, 
	\REM{
	we can decide in $O(nk^2)$ time whether there is a polygonal curve $Q$ through $S$ 
	such that $\distF(P, Q) \lee \eps$, for a given $\eps \gee 0$. }	
	a polygonal curve $Q$ through $S$ of size $O(\min\set{n,k})$ minimizing $\distF(P, Q)$ 
	can be computed in $O(nk^2 \log (nk))$ time. 
	Then we proved that if curve $Q$	is forced to visit every point in the pointset, the problem becomes NP-complete. It is interesting to study special cases of 
	this problem when the input is a specific 
	type of curve, e.g., an $xy$-monotone convex curve.
	In the following, we describe the difficulty in 
	that problem instance, and we provide a potential polynomial time solution 
	for the decision problem, based on the algorithm in Chapter \ref{ch:StayClose} of this thesis.

	\clearpage
	Given an  $xy$-monotone convex curve $P$, a pointset $\pset$
	and distance $\eps \ge 0 $ as input, 
	we call a polygonal curve $Q$ {\em feasible}, if 
	 $Q \in Curves(S)$ and	$\distF(P,Q) \le \eps$ 
	(Curves(S) was defined before in Definition \ref{def:curves}, 
	page \pageref{def:curves}).
	The goal is to decide whether a feasible curve $Q$ can be built in polynomial time 
	through $\pset$ or not. 
	To solve the decision problem, we first run Algorithm 
	\ref{alg:decCCCG11} from Chapter \ref{ch:StayClose} for $(P,S, \eps)$.	
	The output of that 	algorithm  is the reachability sets 
	$\R_1, \R_2, \dots ,\R_{n}$ where each $\R_i$ maintains 
	the reachable points at cylinder $C_i$.  
	
	



\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\columnwidth]{figs/ForwBack}
	\caption{ $u^j \forw v^j$,	$u^j \forw w^k$,	$v^j \not \forw z^k$,	$x^i \not \forw v^j$,  $x^i \see v^j$, $x^i \see z^k$,  
	 $v^j \see z^k$}
	\label{fig:Forw}
	
\end{figure}
	
	
	
	
	We introduce some notation. 
	Let $\lme{i}$ denote the leftmost entry point of cylinder $C_i$.
 	For any reachability set $\R_i$, $ 1\le i < n$,  let $Next(\R_i)$ 
	denote the next non-empty 		reachability set after $\R_i$
	which has some $\Good$ or $\SemiBad$ points or both.  
	Since a point $u \in \pset$ may belong to more than one reachability set, 
	we denote,	by $u^i$,  an instance of $u$ in reachability set $\R_i$.	 
	
	Consider a point $u$ in $\R_i$ and a 		point $v$ in $\R_j$, $i\le j$. 
	Let $u'$ be the leftmost point on $P_i$	such that $\|uu'\| \le \eps$ 
	and let $v'$ be the rightmost point on $P_j$
	such that $\|vv'\| \le \eps$.
	Furthermore, let $P'$ be a subcurve of $P$,
	starting at $u'$  ending at $v'$.
	By $u^i \forw v^j$, we mean $\distF(\Dir{uv},P') \le \eps$.
	% Let $u$ be a point in $\R_i$ and $v$ be a point in $\R_j$, $i \le j$. 
	Furthermore, we say $u^i$ reaches 	$v^j$, 
	and denote it by $u^i\see v^j$, if $u^i \forw v^j$ or
	  a sequence of $m \ge 1$ points 
	$w_1 \in \R_{k_1}, w_2 \in \R_{k_2}, w_3 \in \R_{k_3}, 
	..., w_m \in \R_{k_m}$, 
	$1 \le k_1 \le k_2 \dots k_m \le m$, can be found,
	such that $u^i \forw w_1^{k_1}$, $w_1^{k_1} \forw w_2^{k_2}$, $w_2^{k_2} \forw w_3^{k_3}$ $\dots $  $w_m^{k_m} \forw v^j$
	(see Figure \ref{fig:Forw} for some examples).
	Informally, $u^i \forw v^j$ 
	means $u^i$ can reach $v^j$ directly by 
	taking edge $\Dir{uv}$, 
	and $u^i \see v^j$ means 
	that $u^i$ can reach $v^j$ directly, or indirectly via another point.
	Now notice that points in any reachability set $\R_i$ 
	can be categorized into three groups with respect
	to reaching to points in next cylinders, as the following definition shows.
	
	

	



\begin{definition} 
	\label{def:typeofPoints}
	Let $u$ be a point in $\R_i$ and let $\R_j = Next(\R_i)$. Then, we call $u$
	%\begin{itemize}
	
	(i) $\Good$ point at $C_i$: if $u^i \see \lme{j}$

	(ii) $\SemiBad$ point at $C_i$: 
	if $u^i \nsee \lme{j}$ but $\exists v \in \R_k$, $j \lee k$:  
	$u^i \rightarrow v^k $ %and $v^k \not \rightarrow \lme{j}$
	(see Figure \ref{fig:types})
	
	(iii) $\Bad$ point at $C_i$: if:
	$\nexists v \in \R_k$, $j \le k$: $u^i \see v^k$
	(see Figure \ref{fig:types})	
	%\end{itemize}
	
\end{definition}




\begin{lemma} \label{lemma:NoCurvePreCond}
No feasible curve exists through $S$ if:

$\exists u \in S$	not in any $\R_{i}$, $1\le i \le n$, or

$\R_{n} \cap \CB(t,\eps) = \emptyset$ , or

$\exists u \in \pset$ s.t. $\forall \R_i, u\in \R_i: u$ is $\Bad$ point at $C_i$ 
\end{lemma}


\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{figs/RedYellow}
	\caption{(a,b) Point $u$ is a $\SemiBad$ point at $C_i$ 
(c) Point $u$ is a $\Bad$ point at $C_i$.}
	\label{fig:types}
\end{figure}	
	

	
By $\A{i}$ and $\B{i}$, we
denote the set of $\Good$ and $\SemiBad$ points at $C_i$, respectively.
Clearly if a point $u$ exists in $\pset$, which 
is of $\Bad$ at all cylinders at which $u$ is reachable, 
%$\exists u \in \pset$ s.t. $\forall \R_i, u\in \R_i: u$ is $\Bad$ point at $C_i$, 
then no feasible curve can be built through $S$.






Main difficulty of the decision problem arises due to $\SemiBad$ points, because of 
their following property. 
Imagine point object $\CO_P$, which is
walking on curve $P$ from 
$s$ to $t$, is now on line segment $P_i$
and it is about to move from $P_i$ to $P_{i+1}$.
%Let $\R_j$ be $Next(\R_i)$.
%First, assume that every point in $\R_i$ 
%is of $\Good$ at $C_i$. In this case, 
%we can visit all points in $\R_i$ and 
%stay in $\eps$-distance to
%object $\CO_P$ while it moves to the next line segments along $P$.
%Now 
Assume that there are some $\SemiBad$
points at $C_i$.	
Observe that in this case, 
there are two ways to stay in $\eps$-distance to $\CO_P$
(see Figure \ref{fig:TypeBProperty} for an example): 
either we have to skip  $\SemiBad$ points at $C_i$, or, 
we have to visit them here and instead, 	
skip some points in next cylinders.  

If every point in all reachability sets 
is of $\Good$, one can process those sets
one by one, in order, and easily construct a feasible curve.
%It remains to consider the case where $\B{i}$ is non empty for some $i$. 





To describe our decision algorithm, 
we define function $\LP(u^i)$ as follows.
Let $u$ be a point in $\R_i$. Imagine 
all sets $\R_k$, $i<k$, which have a point $v$
such that $u^i \forw v^k$. Among all such $\R_k$,
let $\R_j$ be the one with the smallest index.
Let $V$ be the subset of $\R_j$ 
which contains all such $v$ points in $\R_j$.
Then, $\LP(u^i)$ is equal to  
 $q^j$ where $ q= \min_{v \in V}{\Left(P_j[v])}$.
Obviously, for every point $u \in \A{i}$, $\LP(u^i) = \lme{Next(\R_i)}$.


Let $u$ be a $\SemiBad$ point at cylinder $C_i$
and let $w^k$ be $lp(u^i)$.
Furthermore, let $\Rivals(u^i)$ denote 
set of points in $\R_j$, $ i < j \le k$,
which will be skipped, if an object visits point 
$u$ at $C_i$ and then takes edge $\Dir{uw}$ 
to stay in $\eps$-\Frechet distance to $\CO_P$.
%when  $\CO_P$ is on $P_i$ and wants to move to the
%next lines segments along $P$. 
%We call 
%those points, {\em rivals} of $u^i$, and denote them by
%$\Rivals(u^i)$.
For an example, see Figure \ref{fig:TypeBProperty}, where $\Rivals(u^i)=\{v^{i+1},w^{i+1},z^{i+1}\}$. 

\begin{lemma}
Given two points $u$ and $v$ in $\B{i}$, $\LP(u^i) = \LP(v^i)$
and $\Rivals(u^i) = \Rivals(v^i)$.
\end{lemma}

\begin{proof}
Let Tube($P$) be the union of all cylinders 
$\CC(\PolSeg_i, \eps)$, $1 \le i \le n$.
We define two curves $P'$ and $P''$
with respect to $P$ as follows.
Imagine a point object $\CO_P$ walks on $P$
from the starting to the ending point of $P$.
Suppose another point object $\CO_P'$,
which wants to  stay always in exact distance $\eps$ to $\CO_P$,
and walks with the same speed as $\CO_P$. 
Then, $\CO_P'$ can follow (or walk) two curves,
which we refer to them as $P'$ and $P''$.
From a view of a point within 
Tube($P$), one of those curves 
is convex and the other one is concave
(because $P$ is a convex curve).
Let $P'$ be the concave one 
(see Figure \ref{fig:typeBVisibility}).
Let $\ell_u$ denote the ray from point $u\in \pset$
tangent to curve $P'$ (in direction of $P'$).
Notice that when $u$ is a \SemiBad~point at 
a cylinder, there must be a bending point 
at a vertex on curve $P$ after that cylinder 
and therefore, we can always draw $\ell_u$.
Let $B(\ell_u)$ denote the side of line $\ell_u$
where $P'$ lies and $T(\ell_u)$
denote the other side of that line.  



\begin{figure}[t]
	\centering
	\includegraphics[width=0.6\columnwidth]{figs/typeBissue2}
	\caption{Illustration of Observation
	\ref{obs:typeBpoints} }
	\label{fig:typeBVisibility}
\end{figure}



Assume w.l.o.g., that  $\Left(P_i[u])$ 
is before $\Left(P_i[v])$ on $P_i$. 
Furthermore, let $\R_j$
be the $Next(\R_i)$ and let
$w$ be a point in $\R_k$ s.t.  $u^i \forw w^k$, 
$i < j \le k$. 
Then, $v^i \see w^k$.



Draw lines $\ell_u$ and $\ell_v$.
If point $v$ lies on $T(\ell_u)$,
then because of the convexity of $P$, 
$v^i \forw w^k$ (see Figure \ref{fig:typeBVisibility}).

Now suppose that $v$ is located on $B(\ell_u)$. 
Consider point $w$. If that point is located 
on $T(\ell_v)$, then again by 
convexity of $P$, $v^i \forw w^k$. 
If not, because $v$ is a $\SemiBad$ point at $C_i$,
a point $z \in \R_m$ exists such that $v^i \forw z^m$, $i<m$.
Now it is clear that $m \le k$ 
because  $v$ is located on $B(\ell_u)$ side of $\ell_u$
and $\Left(P_i[u])$ is before $\Left(P_i[v])$ on $P_i$.
Thus,  $z^m \forw w^k$ and
therefore, $v^i$ reach $w^k$ via $z^m$
($v^i \see  w^k$).

 
 
 
 


For two $\SemiBad$ points $u$ and $v$ 
at $C_i$, $lp(u^i) = lp(v^i)$.

 
 
	



For two $\SemiBad$ points $u$ and $v$ 
at $C_i$, $\Rivals(u^i) = \Rivals(v^i)$.



Assume, w.l.o.g., that $\Left(P_i[u])$
is before  $\Left(P_i[v])$ on $P$.
Let $\R_j$ be the $Next(\R_i)$. 
Then, Observation \ref{obs:typeBpoints} implies 
that if a curve, say curve $\alpha$
(which maintains $\eps$-\Frechet distance to $P$) 
first visits point $u$,
and next, visits point $v$ at $C_i$, then 
$\alpha$ can go to a point, say $u'$, from which 
it can reach points that $v$ reaches as well.
Consequently, the points which $u^i$ and $v^i$ can not 
reach are the same as well. Therefore, $\Rivals(u^i) = \Rivals(v^i)$. 
































\end{proof}



	Let  $P[u]$, $u \in \pset$, denote 
	the set $\{\forall v \in P ~|~  \| uv\| \le \epsilon \}$. 
	Note that $P[u]$ can be a connected or disconnected 
	set of points. 
	For two points $u$ and $v$ in $\pset$, 
	by  $P[u] \lei P[v]$,
	we mean every point in $P[v]$ is located 
	after every point in $P[u]$ on $P$. 
	
	\REM{	
	Now observe that for any $B^i$, $1 \le i <n$,
	a point $u$ in $\B{i}$, a point $v$ in $\Rivals(u^i)$, and $w=\LP(u^i)$,
	if $P[u] \lei P[v] \lei P[w]$, 	 
	then no feasible curve can be built through pointset $\pset$.	
	}
	
	\REM{
	Difficulty in decision arises due to the fact 
	that both $P[u]$ and $P[v]$ can get fragmented and $P[u]$ is not always 
	before $P[v]$ on $P$. 
	We believe that taking the following approach at each 
	cylinder $C_i$ which contains some $\SemiBad$ points,	
	one can decide whether a feasible curve exists through $\pset$ or not.
	
	\vspace{0.2 in}
	Let $u$ be a point in $B^i$, $v \in \Rivals(u^i)$ and $w^k = \LP(u^i)$     
    
   	{\bf if} $(P[v] \lei P[w])$ {\bf and}  $(P[u] \lei P[w])$	{\bf then}				    
    
	\hspace{0.2 in} skip points in $B^i$ and visit points in $\Rivals(u^i)$	
	
	{\bf else} 				
	
	\hspace{0.2 in} visit points in $\B{i}$ \label{l:VisitB}, and skip points in $\Rivals(u^i)$	
	\vspace{0.2 in}				
	}

		





\begin{lemma}
\label{lemma:NoCurveMainCond}
Let $u$ be any point in $\B{i}$
and $v$ be any point in $\Rivals(\B{i})$
and $w$ be $\LP(\B{i})$. 
If $P[u] \lei P[v] \lei P[w]$, 
then no feasible curve exists through $S$.
\end{lemma}

\begin{proof}
This follows from the property of 
$\SemiBad$ points. When $\CO_P$ is at $P_i$, 
one can two choices to stay in 
$\eps$-\Frechet distance to object $\CO_P$ 
(when that object is advance to next line segments):
either skip $\Rivals(\B{i})$ by taking an edge from the last point 
in $B_i$ to $lp(\B{i})$, 
or skip points in $\B{i}$ and, visit $\Rivals{\B{i}}$ instead.
Taking the first choice, we can not visit $v$ anymore
because $\CO_P$ has moved to a point after $P[v]$.
Similarly,  taking the second choice, 
we can not visit $u$ anymore because 
$\CO_P$ has moved to a point after $P[u]$.

\end{proof}					




\begin{figure}[t]
	\centering
	\includegraphics[width=0.55\columnwidth]{figs/PathAB2}
	\caption{Point $u$ is a $\SemiBad$ point at cylinder $C_i$. When object $\CO_P$, 
	walks from $P_i$ to $P_{i+1}$, one could either take path $\langle aub \rangle$ or path $\langle avb \rangle$ to stay in $\eps$-\Frechet distance to $\CO_P$, the object which moves on $P$ }
	\label{fig:TypeBProperty}
\end{figure}	

	

\begin{algorithm} 
\caption {{\sc Decision Algorithm }} 
\label{alg:decFinal}%--KAVEH


\algsetup{indent=1.5em}
\begin{algorithmic}[1]	
\baselineskip=0.9\baselineskip

	\REQUIRE Polygonal chain $P$, %\\
	pointset $\pset$ and distance $\eps$
		
\vspace{0.1 in}
	\STATE Run the decision algorithm in Chapter \ref{ch:StayClose} for $(P, S, \eps)$
		 \label{l:runAlgcccg11}
		 

	\STATE {\bf return} ``{\sc no}" 	if conditions in Lemma \ref{lemma:NoCurvePreCond}  holds
	
%	\vspace{0.1 in}
	
	\STATE $i = 1$
	%\STATE discard from every $\R_i$,   points which are of $\Bad$ at $C_i$ 
	%\label{l:discardtypeCpts}	
 	\WHILE {$i \neq n$ } \label{l:forCylFinalDec}	
		\IF{ $A^i \neq \emptyset$} 
		\STATE visit points in $\A{i}$, let $w^k = \lme{Next(\R_i)}$ \label{l:vistA}
		\ENDIF
	
	  		
		\IF{$B^i \neq \emptyset$}
			%\STATE let $u \in B^i$, $v \in \Rivals(u^i)$ and $w^k = \LP(u^i)$
			\IF {$\exists u\in B^i$ s.t. $P[u]$ is connected }
			\STATE visit  points in $\B{i}$, let $w^k = \LP(u^i)$
			\ELSE 
			\STATE skip points in $B^i$, let $w^k = \lme{Next(\R_i)}$		
			\ENDIF			
				
			\REM{			
			\IF {$(P[u] \lei P[v] \lei P[w])$}
				\STATE {\bf return} ``{\sc no}"
			\ENDIF

			\IF {$(P[v] \lei P[w] ~\AND~ P[u] \lei P[w])  $}		
			
				\STATE skip points in $B^i$, let $w^k = \lme{Next(\R_i)}$
			\ELSE 			
				\STATE  visit points in $\B{i}$ \label{l:VisitB}
			\ENDIF	
			}
		\ENDIF

			\STATE visit $w^k$, i = k \label{l:setNextiFinalDec}
	\ENDWHILE
	\STATE {\bf return} ``{\sc yes}" if $\forall u \in \pset$: $u \in \alpha$
	
	
	%\STATE return  ``{\sc no}" if $\exists u \in \pset : u \notin \alpha$; otherwise, return  ``{\sc YES}" \label{l:eachPointInAlpha}	

\end{algorithmic} 
\end{algorithm} 


		
	




	
	
	
	
\newpage
\begin{lemma}
There exists a feasible curve through $\pset$ iff 
Algorithm \ref{alg:decFinal} returns YES.
\end{lemma}

\begin{proof}
	It is easy to check that when all points
	in every reachability set is of $\Good$, 
	curve $\alpha$ goes through every point in $\pset$ and 
	$\distF(\alpha, P) \le \eps$.
	We show the lemma for the case 
	where some points in a reachability set $\R_i$ are 
 	of $\SemiBad$. %So assume that $\B{i} \neq \emptyset$.
 	
 	Let $u \in B^i$, $w=\LP(u^i)$ and $v \in \Rivals(u^i)$. 	
 	Notice that by 
	Observation $\ref{obs:PwIsConnected}$,
	$P[w]$ is a connected set of points. 
	Two cases occur for $P[w]$ with respect to $P[v]$
	(these cases are depicted in Figure \ref{fig:disconncted}a and	\ref{fig:disconncted}b). 
	In the first one, $P[w]$
	is located after some points of $P[v]$
	and before other points of $P[v]$ on $P$.
	(e.g., see Figure \ref{fig:disconncted}a).
	Note that in that case, $\alpha$ visits points in $\B{i}$
	and goes to $w$ and consequently, skips $\Rivals(\B{i})$. 
	It is sufficient to show that $\alpha$ will visit all points in 
	$\Rivals(\B{i})$.

	
	Let $Q$ be a feasible curve which 
	has skipped points in $\B{i}$ and chosen to 
	visit points in $\Rivals(\B{i})$ here. 
	This implies that $u$ is a point which is 
	reachable at multiple cylinder.  
	Because of Lemma \ref{whenconnctedonlytypeBatLast}, 
	$P[u]$ is a disconnected set of points. 
	
	 
		
	
	
 	
 	\newpage
	In the second case, 
points of $P[w]$ are located after points of $P[v]$, on $P$
(e.g., see Figure \ref{fig:disconncted}b).	
 	
\end{proof}
	
	
	
	
	
	
	
\clearpage
	It would be interesting to study above problem 
	in the case where the input  is
	a non-intersecting curve or a monotone curve. 
	Also, it is interesting to study special cases of All-Points CPM problem  under the
	condition that each point in the pointset can be visited only once.
	
	

==> abstract.tex <==

\begin{abstract}  
\vspace{-0.7 cm}
The \Frechet distance is a well-known  metric to measure similarity of polygonal curves.
In the first part of this thesis, 
%we study some new variants of \Frechet distance problem
%and provide efficient algorithm for solving them:
we introduce a 
new metric called \Frechet distance with speed limits
and provide efficient algorithms for computing it. 
The classical \Frechet distance between two  
curves corresponds to the maximum distance between two point 
objects that traverse the curves with arbitrary non-negative speeds. 
We consider a problem instance in which 
the speed of traversal along each segment of the curves is restricted to be within a specified range. 
This setting is more realistic than 
the classical \Frechet distance setting, specially in GIS applications. 
We also study this problem 
in the setting where the polygonal curves are inside a simple polygon.

%In this thesis, we also propose a new 
%data structure, which can be used 
%in applications involving \Frechet distance.
In the second part of this thesis, 
we present a data structure, called the free-space map, that enables us to solve several variants of the \Frechet distance problem efficiently.
Back in 1995, a data structure was introduced by Alt and Godau, 
called the free space diagram, 
for computing \Frechet distance. 
That data structure is widely used in different applications involving the \Frechet distance.  
Our data structure encapsulates all the information available in the free-space diagram, 
yet it is capable of answering more general type of queries efficiently. 
Given that the free-space map has the same size and construction time as
the standard free-space diagram, it can be viewed as a powerful alternative to it.
As part of the results in Part II of the 
thesis, we exploit the free-space map to improve the long-standing bound for computing the partial \Frechet distance
and obtain improved algorithms for computing the \Frechet distance between two closed curves, and the so-called minimum/maximum walk problem. We also improve the map matching algorithm for the case when the map is a directed acyclic graph.

As the last part of this thesis,
given a point set $S$ and a polygonal curve $P$ in $\IR^d$,
we study the problem of finding a polygonal curve $Q$ through $\pset$,
which has a minimum \Frechet distance to $P$. 
Furthermore, if
the problem requires that curve $Q$ visits every point in 
$S$, we show it is NP-complete. 

%We show that if $Q$ has to 
%visit every point in $\pset$, the problem is NP-complete. 
%At the end, we investigate some 
%special cases of this problem, when the input 
%is a convex monotone chain or a convex polygon.

\end{abstract}


==> ack.tex <==
\noindent {\bf \Large Acknowledgements}

\vspace{0.5in}
I would like to first thank my two supervisors, 
Prof. J\"{o}rg-R\"{u}diger Sack and Prof. Anil Maheshwari. 
I would like to give tremendous thanks to  Prof. Sack
for the support and insight that he has given me 
throughout my degree here at Carleton. 
%He is one of the best in his field and 
%I have tremendous respect for him and his work. 
Prof. Sack, I greatly appreciate your help both academically and financially.
I am happy to have been a part of your research group.



I would like to give many thanks to Anil for the countless hours of 
time that he has made available to me throughout the development of this thesis. 
His many constructive comments and technical advice  have helped me to complete 
this thesis. He has become more of a friend than 
a supervisor for me. Anil, I never forget your helps. 

I would also like to thank
% sincere gratitude 
%and 
%appreciation to 
my co-author and friend, Prof. Hamid Zarrabi-Zadeh, 
for his guidance and assistance in this thesis. 
It was my pleasure to work with an excellent fellow researcher such as Hamid. 
I learned a lot from him. 

I thank the members of my thesis examinations committee 
for their helpful and encouraging comments. 
I would like to highly thank Prof. Helmut Alt for his valuable comments 
and also Prof. Michiel Smid for helpful discussions.

I would like to thank my parents, colleagues and friends for their love
and encouragement for all these years.  

This research was supported by 
National Sciences and Engineering Research Council of Canada 
and SUN Microsystems.	

==> to.tex <==
{\large \emph{ To my father, wish he was here ...} }
